Deep Learning Techniques for Compressive Sensing-Based Reconstruction and Inference -- A Ubiquitous Systems Perspective

Compressive sensing (CS) is a mathematically elegant tool for reducing the sampling rate, potentially bringing context-awareness to a wider range of devices. Nevertheless, practical issues with the sampling and reconstruction algorithms prevent further proliferation of CS in real world domains, especially among heterogeneous ubiquitous devices. Deep learning (DL) naturally complements CS for adapting the sampling matrix, reconstructing the signal, and learning form the compressed samples. While the CS-DL integration has received substantial research interest recently, it has not yet been thoroughly surveyed, nor has the light been shed on practical issues towards bringing the CS-DL to real world implementations in the ubicomp domain. In this paper we identify main possible ways in which CS and DL can interplay, extract key ideas for making CS-DL efficient, identify major trends in CS-DL research space, and derive guidelines for future evolution of CS-DL within the ubicomp domain.

==> tex/glossary.tex <==
\newacronym{ADMM}{ADMM}{Alternating DirectionMethod of Multipliers}
\newacronym{AE}{AE}{Autoencoder} 
\newacronym{AI}{AI}{Artificial Intelligence}
\newacronym{BCS}{BCS}{Bayesian compressive sensing}
\newacronym{BP}{BP}{Basis Pursuit}
\newacronym{BPDN}{BPDN}{Basis Pursuit De-Noising}
\newacronym{CAE}{CAE}{Contractive autoencoder}
\newacronym{CS}{CS}{Compressive Sensing}
\newacronym{CoSAMP}{CoSAMP}{Compressive Sampling Matching Pursuit}
\newacronym{CNN}{CNN}{Convolutional Neural Network}
\newacronym{CRN}{CRN}{Convolutional Residual Network}
\newacronym{CRNN}{CRNN}{Convolutional Recurrent Neural Network}
\newacronym{CT}{CT}{Computed Tomography}
\newacronym{DL}{DL}{Deep Learning}
\newacronym{DAE}{DAE}{Denoising autoencoder}
\newacronym{DBN}{DBN}{Deep Belief Network}
\newacronym{DRN}{DRN}{Deep Residual Network}
\newacronym{ECG}{ECG}{Electrocardiogram}
\newacronym{EEG}{EEG}{Electroencephalogram}
\newacronym{FFNN}{FFNN}{Feed Forward Neural Network}
\newacronym{FOCUSS}{FOCUSS}{Focal Underdetermined System Solution}
\newacronym{GAN}{GAB}{Generative Adversarial Network}
\newacronym{GOMP}{GOMP}{Generalized Orthogonal Matching Pursuit}
\newacronym{IoT}{IoT}{Internet of Things}
\newacronym{IHT}{IHT}{Iterative Hard Thresholding}
\newacronym{IRLS}{IRLS}{Iterative Reweighted Least Squares}
\newacronym{ISTA}{ISTA}{Iterative Shrinkage/Thresholding Algorithm}
\newacronym{LASSO}{LASSO}{Least Absolute Shrinkage and Selection Operator}
\newacronym{LSTM}{LSTM}{Long Short-Term Memory}

\newacronym{MLP}{MLP}{Multi Layer Perceptron}
\newacronym{MP}{MP}{Matching Pursuit}
\newacronym{MR}{MR}{Measurement Rates}
\newacronym{MRI}{MRI}{Magentic Resonance Imaging}
\newacronym{NN}{NN}{Neural Network}
\newacronym{NSP}{NSP}{Null Space Property}
\newacronym{OMP}{OMP}{Orthogonal Matching Pursuit}
\newacronym{RIP}{RIP}{Restricted Isometry Property}
\newacronym{RNN}{RNN}{Recurrent Neural Network} 
\newacronym{SAE}{SAE}{Sparse autoencoder}
\newacronym{SDAE}{SDAE}{Stacked Denoising Autoencoder}
\newacronym{StOMP}{StOMP}{Stagewise Orthogonal Matching Pursuit}
\newacronym{UAV}{UAV}{Unmanned Aerial Vehicles}
\newacronym{UWB}{UWB}{Ultra Wideband}
\newacronym{VAE}{VAE}{Variational autoencoder}
\newacronym{WSN}{WSN}{Wireless Sensor Network}

==> tex/lessons.tex <==
\section{Discussion and Guidelines}
\label{sec:lessons}

% formalize some domains

The recent advances in the CS-DL domain have fundamentally influenced all the blocks in the signal processing chain, from acquisition, compression, transmission, recovery, to inference. Engineering practice in many important areas has been changed by applying the new paradigm. Examples include fast MRI acquisition, image denoising, speech recognition, as well as recommendation systems.

In \textit{the MRI domain}, the DL techniques for CS proved to be able to reduce the scanning time and in the same time to improve the image reconstruction quality.
Various deep learning-based methods have been proposed for MRI, in the past decade. Some of these methods, use deep neural networks to learn the traditional optimization algorithms, by unrolling them ~\cite{sun2016deep,yang2017admm,zhang2020deep}.
Another category of deep learning methods uses deep networks to mitigate noise and aliasing artifacts in the MRI reconstruction. SDAE \cite{majumdar2015real}, CNNs \cite{wang2016accelerating}, residual networks \cite{7950457,han2018deep,sun2018compressed,ouchi2020reconstruction}, or GANs \cite{mardani2017deep, yu2017deep} were successfully validated as suitable architectures for CS MRI and have all shown great potential, outperforming conventional CS techniques for undersampled MRI.
The main advantage of CS-DL methods in MRI lies in the capability of a DNN to capture and make use of the patterns learned within the data in both image and frequency domain, to improve the quality of the reconstruction which is of high importance for medical diagnosis. In this process of reconstruction, the deep-learning based CS solutions go beyond the standard metrics that are usually used for mathematically evaluating the quality of an image, and emphasize more on the anatomical or pathological details.
Also, by shifting the computational efforts to an offline training stage, CS-DL algorithms for MRI are able to provide a fast reconstruction, up to real-time, which is also crucial in clinical practice.
However, a large amount of data  needs to be available to avoid over-fitting in the learning process. The collection of large, high quality, MRI datasets can be challenging, due to patient privacy concerns, among other things. In addition, since the data used for training a certain model becomes an essential component that defines its performance, it is difficult to compare different approaches if the training data is not publicly available. In this regard, a recent solution proposed ~\cite{shin2018medical} was to generate synthetic abnormal MRI images with brain tumors by training a GAN. This approach can overcome the issues of the lack of data for training or that of having imbalanced medical imaging datasets, which was limiting the training of deep learning methods. Another interesting approach was the one in \cite{zhao2020reference} that leverages the Deep Image Prior (DIP) \cite{ulyanov2018deep} framework, for solving imaging inverse problems without pre-training, by using a CNN, initialized with random parameters, and only random noise is prepared as the network input.

As far as \textit{biomedical uni-dimensional signals} (such as EEG or ECG) are concerned, CS-DL methods are used to lower the power consumption and to provide real time execution, with respect to the classical approach. For example, the work in \cite{majumdar2015real}, uses a stacked autoencoder (SAE), for reconstructing the ECG compressed samples, and manages to achieve real time reconstruction. 
Shrivastwa et al. ~\cite{shrivastwa2018fpga} uses a MLP network for ECoG (Electrocorticography) signals compression and reconstruction.
In \cite{singhal2017semi}, the authors go a step further and directly classify ECG and EEG signals in their compressive measurements space, achieving satisfying results with minimal computation, by skipping the reconstruction phase. 
Mangia et al.~ \cite{9044777} uses support identification through DNN-based oracles, to first guess which components are non-zero in the sparse signal to recover, and then compute their magnitudes, thus decreasing the complexity of the computation.

In the field of \textit{Wireless Sensor Networks (WSNs)}, CS-DL based techniques are motivated by not only the sparsity of the signals, but also by the requirement of efficiency in processing in terms of energy consumption and communication bandwidth. Moreover, the compressive measurements are transmitted over wireless channels, so the impact of channel noise and fading on reconstruction are important factors to be taken into consideration.
Some of the most important contributions in the field of CS-DL based methods for WSN are the WDLReconNet, and Fast-WDLReconNet networks ~\cite{lu2019wdlreconnet}, validated for the transmission of remote sensing images.
An interesting fact in this model is that the number of parameters in the denoising layer accounts for about 94\% of the total number of parameters in the CNN, underlying the impact of the noise on the transmitted data. 
Energy efficiency is another major aspect in WSN and quantization proved to be able to ensure an efficient wireless transmission~\cite{7560597}. 

% towards hardware co-design
Despite extensive research, analog to digital conversion remains a bottleneck in applications that requires high sampling rates and high bandwidth. This leads to high power and high cost that blocks the development of new technologies. Developing signal specific methods of analog to digital conversion may provide a way forward.

CS-DL real-world implementations have to meet the requirements of the hardware architectures that are small size, low cost and low power, while also enabling fast acquisition and recovery of information at significantly reduced bandwidth.
These objectives will require the \textit{co-design of the digital components, together with the CS-DL algorithms}. 
A few CS-based solutions have been proposed so far in the literature \cite{zhang2014efficient,shoaran2014compact,pareschi2015hardware,cambareri2015case,mangia2017zeroing} for integrated CS hardware design. 
The co-design of the hardware together with the acquisition and the reconstruction algorithms, has the potential to maximize the performance while also reducing the hardware complexity \cite{7192741}. 

However, there is currently a lack of implementations involving deep learning compressive sensing and hardware co-design. To the best of our knowledge, the work in ~\cite{shrivastwa2018fpga}, targeting a FPGA implementation of a deep neural network for ECoG signals compression and reconstruction is one of the few such works.
Without doubt, the successful development of implementation-friendly algorithms and architectures would accelerate the expansion of the CS field and lead to the commercialization of CS based systems.
In the future, it is expected to see more hardware implementations of CS-DL with built in hardware.



